Broadband and Large-Multimode Quantum Optical Storage with Rare-Earth Ions in Solids

Broadband quantum memory devices are essential elements for future quantum networks. Here we propose a broadband quantum memory scheme called Hole Anti-hole Grating Echo Memory (HAGEM) for rare-earth ions in solids, which can be implemented with most of the present rare-earth ions hosted in various types of solids. Using HAGEM, a quantum memory device with one billion temporal modes per second can be developed with current available technologies. To validate the memory protocol, we conducted some proof-of-concept experiments. We provide a Eu$^\text{{3+}}$ molecular complex with special hyperfine level structures of which the hyperfine level separations are in a specific mathematical correlation that can be obtained by harnessing chemical engineering. Using the proposed memory protocol and material, we experimentally demonstrate a single-mode quantum optical storage efficiency of 14.9% and a memory bandwidth of 200MHz, which can easily be extended to a few GHz. In addition, a multi-mode storage of four temporal modes is achieved with a storage efficiency of 1.3%. Broadband & large-multimode quantum memory device with a long storage time enabled by HAGEM integrating with the current available entangled photon pair source and tunable delay lines, a quantum repeater network with an entanglement distribution rate on the order of 1kHz - 10kHz can be created with a communication distance around 100km. This will greatly facilitate the development of quantum networks in near future.

==> crystal_field_model.tex <==
\providecommand{\sampleTMHD}{\ensuremath{\mathrm{Eu^{3+}(TMHD)_3(phen)}}}
\providecommand{\sampleBA}{\ensuremath{\mathrm{Eu^{3+}(BA)_4(pip)}}}
\ifdefined\angstromunit\else
  \DeclareSIUnit\angstromunit{\text{\AA}}
\fi

% \section{Crystal-field and hyperfine model}
% \label{sec:cf-model}

The optical and hyperfine measurements described in the previous sections
provide complementary information about the Eu$^{3+}$ electronic and nuclear
wavefunctions. To connect these observables within one description, we
constructed a Hamiltonian for the Eu$^{3+}$ molecular platform that links the
molecular coordination structure to the crystal-field levels, the zero-field
hyperfine splittings of the $^7F_0$ and $^5D_0$ states, and the measured
branching ratios between their hyperfine levels. The formalism follows the
complete Eu$^{3+}$ crystal-field treatment of Smith \textit{et al.}
\cite{smith2022complete}. Matrix elements were generated with M.~F. Reid's
LinuxEMP programs \cite{reidLinuxEMP} and assembled, diagonalized, and fitted
with PyCF \cite{horvath2016high}.

\subsection{Full system Hamiltonian}

The Hamiltonian for the $4f^6$ configuration is
\begin{equation}
H=H_{\mathrm{FI}}+H_{\mathrm{CF}}+H_{\mathrm{Z}}
  +H_{\mathrm{MD}}+H_Q^{4f}+H_Q^{\mathrm{lat}},
\label{eq:total-hamiltonian}
\end{equation}
where the terms describe the free ion, crystal field, electronic and nuclear
Zeeman interactions, magnetic-dipole hyperfine interaction, and the
$4f$-electron and lattice contributions to the nuclear electric-quadrupole
interaction, respectively. The present spectra were measured at zero magnetic field, so
$H_{\mathrm{Z}}=0$ in every fit reported here.

The free-ion Hamiltonian was written in the standard effective-operator form
\begin{align}
H_{\mathrm{FI}}={}&E_{\mathrm{avg}}
 +\sum_{k=2,4,6}F^k f_k+\zeta_{4f}A_{\mathrm{SO}}
 +\alpha L(L+1)+\beta G(G_2)+\gamma G(R_7) \notag\\
&+\sum_{i=2,3,4,6,7,8}T^i t_i
 +M_{\mathrm{tot}}m_{\mathrm{tot}}
 +P_{\mathrm{tot}}p_{\mathrm{tot}}.
\label{eq:free-ion-hamiltonian}
\end{align}
Here, $E_{\mathrm{avg}}$ is the configuration-average energy, $F^k$ are the
electrostatic Slater parameters, and $\zeta_{4f}$ is the spin--orbit coupling
parameter. The composite Marvin operator $m_{\mathrm{tot}}$ represents the
spin--spin and spin--other-orbit corrections, whereas $p_{\mathrm{tot}}$ is
the composite operator for the electrostatically correlated spin--orbit
correction. The remaining operators describe smaller electrostatic,
configuration-interaction, and relativistic corrections.

For an even-parity $4f^6$ configuration, the crystal-field Hamiltonian
contains only $k=2$, 4, and 6. In the full spherical-tensor notation,
\begin{equation}
H_{\mathrm{CF}}=\sum_{k=2,4,6}\sum_{q=-k}^{k}B_q^k C_q^{(k)},
\qquad
B_{-q}^k=(-1)^q\left(B_q^k\right)^*.
\label{eq:cf-full}
\end{equation}
The second relation enforces Hermiticity. PyCF therefore requires only the
non-negative-$q$ members, which were assembled as
\begin{equation}
H_{\mathrm{CF}}=\sum_{k=2,4,6}\left[
B_0^kC_0^{(k)}+\sum_{q=1}^{k}\left\{
B_q^kC_q^{(k)}+\left[B_q^kC_q^{(k)}\right]^\dagger
\right\}\right].
\label{eq:cf-pycf}
\end{equation}
Thus $B_0^k$ is real, while $B_q^k=B_q^{k,\mathrm{R}}+
iB_q^{k,\mathrm{I}}$ for $q>0$. Both Eu sites have $C_1$ local symmetry.
Consequently, summing the real $q=0$ terms and the real and imaginary
components for every $q>0$ over $k=2$, 4, and 6 gives 27 symmetry-allowed
real crystal-field degrees of freedom.

The general Zeeman term retained for future field-dependent calculations is
\begin{equation}
H_{\mathrm{Z}}=\mu_{\mathrm{B}}\mathbf{B}\!\cdot\!
\left(\mathbf{L}+g_s\mathbf{S}\right)
-g_n\mu_{\mathrm{N}}\mathbf{B}\!\cdot\!\mathbf{I}.
\label{eq:zeeman-hamiltonian}
\end{equation}
For $^{151}\mathrm{Eu}^{3+}$, $I=5/2$. The magnetic-dipole hyperfine
operator was written as \cite{smith2022complete}
\begin{equation}
H_{\mathrm{MD}}=a_l\sum_i\mathbf{N}_i\!\cdot\!\mathbf{I},
\qquad
\mathbf{N}_i=\mathbf{l}_i-\sqrt{10}
\left(\mathbf{s}_iC_i^{(2)}\right)^{(1)},
\label{eq:magnetic-hyperfine}
\end{equation}
and the $4f$ electric-quadrupole interaction was written in the same
unit-tensor convention as Smith \textit{et al.}: \cite{smith2022complete}
\begin{equation}
H_Q^{4f}=\frac{E_Q}{2}
\left[\frac{(I+1)(2I+1)(2I+3)}{I(2I-1)}\right]^{1/2}
U_n^{(2)}\!\cdot\!U_e^{(2)}.
\label{eq:electronic-quadrupole}
\end{equation}
For the lattice nuclear-quadrupole interaction, we use the definition given
by Smith \textit{et al.}, \cite{smith2022complete}
\begin{equation}
H_Q^{\mathrm{lat}}=\sum_{q=-2}^{2}N_q^2
\left(U_n\right)_q^{(2)},
\label{eq:lattice-quadrupole}
\end{equation}
where $U_n^{(2)}$ acts on the nuclear wavefunction and the coefficients
$N_q^2$ scale the five components of the lattice electric-field gradient.
Hermiticity requires $N_{-q}^2=(-1)^q(N_q^2)^*$; consequently, $N_0^2$ is
real, whereas $N_1^2$ and $N_2^2$ are complex, giving five independent real
parameters. The matrix elements for this interaction were also generated
with LinuxEMP.

\subsection{Matrix-element construction and free-ion reference}

A complete $4f^6$ free-ion basis was first constructed in LinuxEMP, and the
reference free-ion Hamiltonian was diagonalized using the parameters in
Table~\ref{tab:free-ion-generation}. These are the mean Eu$^{3+}$ free-ion
parameters reported by Smith \textit{et al.}\cite{smith2022complete} and are
the exact values supplied when generating the reference eigenvectors. The
configuration-average coefficient $E_{\mathrm{avg}}$ was not required at
this stage because it adds only a constant energy shift and does not change
the eigenvectors.

\begin{table}[H]
\centering
\caption{Free-ion parameters, in \si{cm^{-1}}, used to generate the reference
Eu$^{3+}$ free-ion eigenvectors and operator matrices.}
\label{tab:free-ion-generation}
\small
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{@{}rrrrrrrrrrrrrrr@{}}
\toprule
$F^2$ & $F^4$ & $F^6$ & $\alpha$ & $\beta$ & $\gamma$
& $T^2$ & $T^3$ & $T^4$ & $T^6$ & $T^7$ & $T^8$
& $\zeta_{4f}$ & $M_{\mathrm{tot}}$ & $P_{\mathrm{tot}}$\\
\midrule
82786 & 59401 & 42644 & 19.80 & $-617$ & 1460
& 370 & 40 & 40 & $-330$ & 380 & 370 & 1332 & 2.38 & 303\\
\bottomrule
\end{tabular}%
}
\end{table}



The resulting eigenvectors were used to generate matrices for the free-ion
and crystal-field operators, as well as the nuclear-expanded magnetic-dipole,
electronic-quadrupole, and complete rank-two lattice-quadrupole interactions.
The generated matrices were converted to text form and imported into PyCF;
the LinuxEMP inputs and converted matrices were retained as the calculation
record. The lowest 30 free-ion multiplets were retained, corresponding to 272
electronic states. Including the six
$m_I=-5/2,-3/2,\ldots,5/2$ nuclear basis states gives a
1632-dimensional hyperfine Hamiltonian.

PyCF combined these fixed operator matrices with the parameter coefficients.
Only the coefficients were varied during fitting; the basis and operator
matrices remained unchanged. The values in
Table~\ref{tab:free-ion-generation} therefore define the reference basis used
during matrix generation rather than fixing every subsequent fit coefficient.
In particular, $F^4$ and $\zeta_{4f}$ were varied during the optical
refinement.

\subsection{Point-charge initialization}
\label{sec:point-charge}

The low $C_1$ symmetry makes an unconstrained fit from arbitrary
crystal-field coefficients unreliable. A structure-based starting point was
therefore calculated from each Crystallographic Information File (CIF)
structure by adapting published point-charge formalisms for lanthanide crystal fields
\cite{li2024elucidating,dun2021effective}. We used the
Racah-normalized spherical harmonics
\begin{equation}
C_q^{(k)}(\theta,\phi)=
\sqrt{\frac{4\pi}{2k+1}}Y_{kq}(\theta,\phi).
\label{eq:racah-normalization}
\end{equation}
For donor atom $i$ with effective charge $Q_i$, Eu--donor vector
$\mathbf r_i$, distance $R_i=|\mathbf r_i|$, and angles
$(\theta_i,\phi_i)$, the geometry moments and initial crystal-field
coefficients were evaluated as
\begin{align}
A_q^k&=\sum_i\frac{Q_i(-1)^q
C_{-q}^{(k)}(\theta_i,\phi_i)}{R_i^{k+1}},
\label{eq:geometry-moment}\\
B_q^{k,\mathrm{PC}}&=K_{\mathrm C}
\langle4f|r^k|4f\rangle A_q^k,
\label{eq:point-charge}
\end{align}
where
\begin{equation}
K_{\mathrm C}=14.3996454784255~\si{eV.\angstromunit}
\times8065.544005~\si{cm^{-1}.eV^{-1}}
=116140.974263~\si{cm^{-1}.\angstromunit}.
\label{eq:coulomb-conversion}
\end{equation}
Equation~\eqref{eq:geometry-moment} is a spherical-multipole projection of
the discrete ligand charge distribution. The radial weighting is
$R_i^{-(k+1)}$, so $A_q^k$ describes the geometry and angular character of
the ligand field, while the radial expectation value and Coulomb conversion
factor produce $B_q^{k,\mathrm{PC}}$. The identity
$(-1)^qC_{-q}^{(k)}=C_q^{(k)*}$ was used in the numerical evaluation. Only
$q\geq0$ was stored, with negative-$q$ coefficients supplied by the
Hermiticity relation in Eq.~\eqref{eq:cf-full}.

The Eu$^{3+}$ radial moments were taken from the Freeman--Watson free-ion
tabulation as implemented in PyCF \cite{freeman1962theoretical}:
\begin{equation}
\langle r^2\rangle=0.2626667523~\si{\angstromunit^2},\quad
\langle r^4\rangle=0.1782395051~\si{\angstromunit^4},\quad
\langle r^6\rangle=0.2562581307~\si{\angstromunit^6}.
\label{eq:radial-moments}
\end{equation}
Odd ranks were not included because the Hamiltonian was restricted to the
even-parity $4f^6$ configuration.

The CIF structures were read without primitive-cell reduction. For the first
symmetry-equivalent Eu site, all oxygen or nitrogen neighbours within
\SI{2.8}{\angstromunit} were sorted by Eu--donor distance, and exactly eight
donors were retained. The first shell of \sampleBA{} contains eight oxygen donors
with distances from \SI{2.353427}{\angstromunit} to
\SI{2.438445}{\angstromunit}. The shell of \sampleTMHD{} contains six oxygen
donors at \SIrange{2.313241}{2.387742}{\angstromunit} and two nitrogen donors at
\SI{2.621514}{\angstromunit} and \SI{2.621572}{\angstromunit}. Each donor
was assigned the provisional effective charge $Q_i=-3/8$, so that the shell
charge sums to $-3e$. This is an initialization convention, not an
atom-resolved oxidation-state or population-analysis assignment.

A fixed local Cartesian frame was chosen for each structure and used
consistently for the point-charge calculation and fitting. This choice fixes
the orientation of the complex $B_q^k$ coefficients but neither adds a term
to the Hamiltonian nor imposes a site symmetry. All 27 allowed coefficients
were calculated. Their signs, relative magnitudes, and orientation supplied
physically informed starting conditions; they were not treated as a final
electrostatic description of covalency or charge redistribution and are
therefore not tabulated.

\subsection{Spectral constraints and fitting procedure}
\label{sec:fitting-procedure}

The spectrum fitted for \sampleTMHD{} was read from
Main Texts Fig. 2(d) ; the spectrum fitted for \sampleBA{}
was read from the reference paper Fig. 1(b) \cite{serrano2022ultra}. For display and peak screening, each trace was
baseline corrected by subtracting its second intensity percentile and was
independently normalized to unit maximum. The fitted observables were peak
centres rather than spectral intensities.

For \sampleTMHD{}, a nine-point, third-order Savitzky--Golay copy of the
normalized trace was used only to screen candidate peaks. Peaks were located
with a minimum separation of four samples and a minimum width of one sample.
The primary prominence threshold was the larger of ten times the
median-absolute-deviation noise estimate and 0.005 normalized intensity; a
secondary threshold equal to the larger of six times the noise estimate and
0.003 flagged weak candidates. For \sampleBA{}, the raw-data screen used a
minimum separation of \SI{0.25}{\nano\meter} and prominence thresholds of
0.001, 0.005, and 0.005 in the $^7F_0$, $^7F_1$, and $^7F_2$ windows,
respectively. The $^7F_0$ and $^7F_1$ centres were refined with Lorentzian
components on a linear background. The five listed \sampleBA{} $^7F_2$
centres came from the working five-component decomposition, but only the first
two clearly resolved components entered the crystal-field objective.

The $^5D_0\rightarrow{}^7F_0$ emission line was used as the reference
transition. If its vacuum wavelength is $\lambda_0$, the energy of a final
$^7F_J$ crystal-field level relative to the lowest $^7F_0$ level was
calculated from
\begin{equation}
E_i=10^7\left(\frac{1}{\lambda_0}-\frac{1}{\lambda_i}\right)
\quad\text{in }\si{cm^{-1}},
\label{eq:wavelength-energy}
\end{equation}
when the wavelengths are in nm. The $^5D_0$ energy relative to the lowest
$^7F_0$ level was taken as $10^7/\lambda_0$.

The fit was performed in stages. First, the free-ion and crystal-field
Hamiltonian was diagonalized using the complete point-charge starting set,
with the hyperfine terms omitted, to obtain the electronic crystal-field
level structure of the $^7F_J$ and $^5D_0$ manifolds. The optical refinement
then allowed only the most influential parameters, $F^4$, $\zeta_{4f}$,
$B_0^2$, $\operatorname{Re}(B_2^2)$, $B_0^4$, and
$\operatorname{Re}(B_4^4)$, to vary; the remaining crystal-field parameters
were retained at their point-charge values. Peak order, the maximum number
of Stark components in each $^7F_J$ manifold, and the stability of the fit
were considered together when assigning the screened features. Only
confidently identified peaks were included in the loss function; weak or
ambiguous features were retained as an external comparison. For
\sampleTMHD{}, several starts around the point-charge solution were used to
reduce dependence on one local minimum and to compare the possible
order-preserving assignments of the unresolved $^7F_2$ level.

The optical parameters were then used to calculate the $^7F_0$ and $^5D_0$
hyperfine manifolds. The magnetic-dipole coefficient, electronic-quadrupole
coefficient, and five real components of the lattice-quadrupole interaction
were refined against the four measured zero-field splittings and the
independent elements of the branching matrix. The selected \sampleTMHD{}
assignment kept its optical parameters fixed during this step. For
\sampleBA{}, a final joint refinement also allowed $B_0^2$ and complex
$B_2^2$ to respond to the hyperfine and branching data while the assigned
optical levels remained constrained. All refinements used bounded nonlinear
least squares. The selected peaks, final level comparisons, and the final
fitted Hamiltonian parameters and their spectroscopic comparison are reported
in the subsequent subsections.

\subsection{Calculation of hyperfine-state branching ratios}

The use of calculated hyperfine transition strengths as constraints on
crystal-field wavefunctions follows earlier work on
$\mathrm{Pr}^{3+}{:}\mathrm{La}_2(\mathrm{WO}_4)_3$
\cite{guillot2010calculation}. For the present Eu$^{3+}$ system, the $^7F_0$
and $^5D_0$ electronic states are singlets, so the relative transition
strengths between their hyperfine states are determined by the overlap of the
nuclear components of their eigenvectors \cite{smith2022complete}. These
components were obtained by projecting each full eigenvector onto the six
$J=0\otimes|m_I\rangle$ basis states and normalizing the result. At zero
field, the six states form three doublets in each manifold. The strength
between ground doublet $i$ and excited doublet $j$ was calculated as
\begin{equation}
S_{ij}=\sum_{\alpha=1}^{2}\sum_{\beta=1}^{2}
\left|\left\langle\Psi_{g,i,\alpha}^{(n)}
\middle|\Psi_{e,j,\beta}^{(n)}\right\rangle\right|^2.
\label{eq:doublet-strength}
\end{equation}
Each ground-state row was then normalized,
\begin{equation}
\mathrm{BR}_{ij}=\frac{S_{ij}}{\displaystyle\sum_{j'=1}^{3}S_{ij'}},
\qquad \sum_{j=1}^{3}\mathrm{BR}_{ij}=1.
\label{eq:branching-ratio}
\end{equation}
Because these observables constrain eigenvectors rather than only
eigenvalues, they provide information not contained in the optical and
hyperfine energies alone.

\subsection{Effective quadrupole projection and decomposition}
\label{sec:q-method}

To separate the physical contributions to the zero-field hyperfine
structure, four calculations were made for each of the $^7F_0$ and $^5D_0$
manifolds while retaining the fitted free-ion and crystal-field coefficients:
\begin{align}
Q_{\mathrm{pq}} &: a_l\ne0,\quad E_Q=N_0^2=N_1^2=N_2^2=0,\\
Q_{4f} &: E_Q\ne0,\quad a_l=N_0^2=N_1^2=N_2^2=0,\\
Q_{\mathrm{lat}} &: N_0^2,N_1^2,N_2^2\ne0,\quad a_l=E_Q=0,\\
Q_{\mathrm{tot}} &: a_l,E_Q,N_0^2,N_1^2,N_2^2\ne0.
\label{eq:q-settings}
\end{align}
Here ``$\ne0$'' means that the coefficient was set to its fitted value.
$Q_{\mathrm{pq}}$ is the effective second-order interaction generated by
magnetic-dipole hyperfine coupling and crystal-field mixing with electronic
states of nonzero $J$; it is not an additional bare term in
Eq.~\eqref{eq:total-hamiltonian}.

For a target manifold, the six eigenstates having the largest summed weight
in the ordered basis
\begin{equation}
\{J=0\}\otimes
\left\{|m_I\rangle:m_I=-5/2,-3/2,-1/2,1/2,3/2,5/2\right\}
\label{eq:nuclear-basis}
\end{equation}
were selected. Let $V$ be the $6\times6$ overlap matrix between this fixed
basis and the selected eigenstates. Its polar decomposition $V=UP$ supplies
the closest unitary mapping $U$ into the fixed nuclear basis. After averaging
the two energies in each zero-field doublet, the trace-free effective
Hamiltonian was formed as
\begin{equation}
H_0=U\,\mathrm{diag}(\bar E_1,\ldots,\bar E_6)U^\dagger,
\qquad
H_{\mathrm{eff}}=H_0-\frac{\operatorname{Tr}(H_0)}{6}\mathbf1.
\label{eq:downfolding}
\end{equation}

The resulting matrix was fitted by linear least squares to the identity and
the complete five-component rank-two nuclear-operator basis generated by
LinuxEMP: $N_{20}$, $\operatorname{Re}N_{21}$,
$\operatorname{Im}N_{21}$, $\operatorname{Re}N_{22}$, and
$\operatorname{Im}N_{22}$. Calibration against the corresponding Cartesian
quadratic spin operators gives a real, symmetric, traceless tensor
$\mathbf Q$,
\begin{equation}
H_Q^{\mathrm{eff}}=\mathbf I\!\cdot\!\mathbf Q\!\cdot\!\mathbf I.
\label{eq:effective-q-tensor}
\end{equation}
For each material and manifold, the principal axes were defined from
$\mathbf Q_{\mathrm{tot}}$, with the largest absolute principal value
assigned to $z$ and the frame made right-handed. Every isolated contribution
was then expressed in this same frame. Following Smith \textit{et al.}
\cite{smith2022complete}, the tensor in the total-tensor principal frame is
written as
\begin{equation}
\mathbf Q=
\begin{pmatrix}
-E-D/3&0&0\\
0&E-D/3&0\\
0&0&2D/3
\end{pmatrix},
\qquad
D=\frac32Q_{zz},\quad E=\frac12(Q_{yy}-Q_{xx}).
\label{eq:d-e-from-q}
\end{equation}
This gives
$H_Q^{\mathrm{eff}}=D[I_z^2-I(I+1)/3]+E(I_y^2-I_x^2)$.
Interchanging the $x$ and $y$ labels reverses the sign of $E$ without
changing the physical Hamiltonian. Both $D$ and $E$ are therefore required
for the present $C_1$ sites. Expressing all isolated tensors in the common
frame of $\mathbf Q_{\mathrm{tot}}$ also makes their scalar components
suitable for an additive comparison.


==> fitted_results.tex <==
\providecommand{\sampleTMHD}{\ensuremath{\mathrm{Eu^{3+}(TMHD)_3(phen)}}}
\providecommand{\sampleBA}{\ensuremath{\mathrm{Eu^{3+}(BA)_4(pip)}}}

\subsection{Optical constraints and assignments}
\label{sec:fit-results}

For \sampleTMHD{}, the possible order-preserving placements of one unobserved
$^7F_2$ component among the four securely observed peaks were tested from the
point-charge starting model. The reported assignment maps the four observed
peaks, in increasing energy order, to components 2--5 and treats component 1
as unobserved. \sampleBA{} uses the original finalized joint fit and is
independent of this \sampleTMHD{} assignment test.

Table~\ref{tab:optical-peaks} lists the centres assigned in the reported fits
and the role of each feature. Figure~\ref{fig:spectral-selection} shows the
corresponding measured spectral regions. The dark curves are the
baseline-corrected, normalized samples, and the lighter traces are the
screening copies described in Section~\ref{sec:fitting-procedure}; neither
spectral intensity trace was fitted by the crystal-field model. For
\sampleTMHD{}, the $^5D_0\rightarrow{}^7F_0$ reference transition, all three
resolved $^7F_1$ peaks, and four $^7F_2$ peaks were retained. In the selected
ordering, the observed $^7F_2$ peaks correspond to components 2--5.
Component 1 is predicted near \SI{609.060}{\nano\meter}, where no convincing
peak is present, and the weak feature near \SI{631.553}{\nano\meter} was
withheld.

For \sampleBA{}, the $^5D_0\rightarrow{}^7F_0$ reference transition, the
three $^7F_1$ peaks, and the first two $^7F_2$ peaks were used as constraints.
Three much weaker $^7F_2$ components from the working spectral decomposition
were retained only for comparison and were not included in the objective
function.

\begin{table}[H]
\centering
\caption{Optical peak centres and their role in the reported crystal-field
fits. ``Predicted'' denotes a calculated level without an assigned
experimental peak.}
\label{tab:optical-peaks}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lllr@{\ }l@{}}
\toprule
Material & Manifold & Component & \multicolumn{1}{c}{Wavelength (nm)} & Role\\
\midrule
\sampleTMHD{} & $^7F_0$ & reference & 580.414965 & used\\
       & $^7F_1$ & 1 & 590.175632 & used\\
       &           & 2 & 591.627603 & used\\
       &           & 3 & 598.332310 & used\\
       & $^7F_2$ & 1 & 609.059748 & predicted, unobserved\\
       &           & 2 & 612.367265 & used\\
       &           & 3 & 617.324661 & used\\
       &           & 4 & 619.942329 & used\\
       &           & 5 & 626.539867 & used\\
       &           & weak feature & 631.552965 & withheld\\
\addlinespace
\sampleBA{} & $^7F_0$ & reference & 580.124880 & used\\
       & $^7F_1$ & 1 & 590.737449 & used\\
       &           & 2 & 592.261992 & used\\
       &           & 3 & 595.001605 & used\\
       & $^7F_2$ & 1 & 612.358000 & used\\
       &           & 2 & 613.083000 & used\\
       &           & 3 & 615.584000 & withheld\\
       &           & 4 & 617.184000 & withheld\\
       &           & 5 & 618.158000 & withheld\\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=\textwidth]{spectral_peak_selection.pdf}
  \caption{Experimental photoluminescence regions used to select the optical
  crystal-field constraints. Dark curves are raw samples after baseline
  correction and normalization; light curves are screening traces. Downward
  triangles mark peaks returned by the automated screen. Teal guides identify
  peak centres used in the fit, amber dashed guides identify weak or tentative
  features withheld from the objective, and the purple dotted guide marks the
  unobserved \sampleTMHD{} $^7F_2$-1 level predicted by the selected
  assignment.}
  \label{fig:spectral-selection}
\end{figure}

\subsection{Crystal-field levels}

Figure~\ref{fig:optical-levels} compares the fitted optical levels with the
experimental constraints. Securely assigned levels are distinguished from
ambiguous features that were withheld from the objective function. For
\sampleTMHD{}, the root-mean-square residual of the fitted optical constraints
is \SI{16.82}{\per\centi\meter}, with a maximum absolute residual of
\SI{25.25}{\per\centi\meter}. This larger residual is retained explicitly as
a limitation of the selected assignment. For \sampleBA{}, the corresponding
values are \SI{1.38}{\per\centi\meter} and
\SI{2.79}{\per\centi\meter}, respectively. These \sampleBA{} statistics were
calculated only from levels included in the objective function. The three weak
$^7F_2$ features were excluded from the loss function and therefore did not
influence the optimization or the quoted residuals; they are shown only as an
external comparison with the final prediction.

\begin{figure}[H]
  \centering
  \includegraphics[width=\textwidth]{optical_level_comparison.pdf}
  \caption{Comparison of experimental and calculated optical crystal-field
  levels for \sampleTMHD{} and \sampleBA{}. Calculated levels are plotted
  above the central axis and experimental features below it. Teal lines denote
  secure constraints included in the fit; amber lines denote ambiguous or weak
  features withheld from the objective. The \sampleTMHD{} panel uses the
  selected assignment described in the text. The broken horizontal scale
  separates the $^5D_0$ transition from the lower $^7F_J$ crystal-field
  levels.}
  \label{fig:optical-levels}
\end{figure}

\subsection{Final Hamiltonian parameters and eigenstates}

Table~\ref{tab:final-parameters} lists the final free-ion, crystal-field, and
hyperfine coefficients for both materials using the notation of
Eq.~\eqref{eq:total-hamiltonian}. Complex coefficients are written as $a+bi$.
The remaining smaller free-ion coefficients were common to both materials and
fixed to the matrix-generation values in
Table~\ref{tab:free-ion-generation}.

\begin{table}[H]
\centering
\caption{Final Hamiltonian parameters for the two Eu(III) molecular
materials. All values are in \si{cm^{-1}}.}
\label{tab:final-parameters}
\small
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular}{@{}lcc@{}}
\toprule
Parameter & \sampleTMHD{} & \sampleBA{}\\
\midrule
$E_{\mathrm{avg}}$ & 64154 & 64154\\
$F^2$ & 83479 & 83479\\
$F^4$ & 59324.829 & 59278.289\\
$F^6$ & 42506 & 42506\\
$\zeta_{4f}$ & 1334.074 & 1301.287\\
\addlinespace
$B_0^2$ & $-407.817$ & $290.909$\\
$B_1^2$ & $0$ & $0$\\
$B_2^2$ & $-226.548$ & $-88.475-0.999i$\\
$B_0^4$ & $2153.302$ & $1392.694$\\
$B_1^4$ & $92.175-19.071i$ & $-9.586-28.388i$\\
$B_2^4$ & $-8.986-20.618i$ & $2.857+4.267i$\\
$B_3^4$ & $51.174-57.520i$ & $-11.273-0.890i$\\
$B_4^4$ & $2021.565+46.817i$ & $-396.331-3.519i$\\
$B_0^6$ & $-38.781$ & $-55.923$\\
$B_1^6$ & $-20.933+5.955i$ & $2.554+7.994i$\\
$B_2^6$ & $-7.656+6.065i$ & $2.013+2.006i$\\
$B_3^6$ & $5.528-11.418i$ & $-4.718+4.377i$\\
$B_4^6$ & $5.461+4.552i$ & $-0.265+0.721i$\\
$B_5^6$ & $4.606+6.958i$ & $0.879+2.256i$\\
$B_6^6$ & $-4.275+3.017i$ & $-3.801+2.172i$\\
\addlinespace
$a_l$ & $0.0200007$ & $0.0250940$\\
$E_Q$ & $-0.0425077$ & $-0.0370611$\\
$N_0^2$ & $0.0046740$ & $-0.0053607$\\
$N_1^2$ & $-0.0006385+0.0017784i$ & $-0.0012118-0.0009873i$\\
$N_2^2$ & $0.0047353+0.0004763i$ & $0.0002371+0.0017993i$\\
\bottomrule
\end{tabular}
\end{table}

The same fitted free-ion and crystal-field parameters were also used to
examine the electronic-state composition before the hyperfine interactions
were introduced. We diagonalized the zero-field electronic Hamiltonian
\begin{equation}
H_{\mathrm{el}}=H_{\mathrm{FI}}+H_{\mathrm{CF}},
\label{eq:electronic-hamiltonian-mixing}
\end{equation}
with the magnetic-dipole hyperfine, electronic quadrupole-hyperfine, and
lattice nuclear-quadrupole terms omitted. For an electronic eigenstate
$\lvert\Psi_n\rangle$, its total weight in the subspace having angular
momentum $J$ was calculated as
\begin{equation}
W_J(\Psi_n)=
\sum_{\alpha}\sum_{M_J=-J}^{J}
\left|
\left\langle\alpha J M_J\middle|\Psi_n\right\rangle
\right|^2,
\qquad
\sum_J W_J(\Psi_n)=1,
\label{eq:j-mixing-weight}
\end{equation}
where $\alpha$ denotes the remaining free-ion labels, including the spin and
orbital term labels. The resulting $J$ compositions of the two optical states
are listed in Table~\ref{tab:j-mixing}.

\begin{table}[H]
\centering
\caption{Calculated $J$ composition of the electronic $^7F_0$ and $^5D_0$
states obtained using the final fitted parameters without hyperfine terms.
All entries are percentages. ``Other'' contains the summed contributions from
all $J$ values other than 0, 2, and 4.}
\label{tab:j-mixing}
\small
\begin{tabular}{llrrrr}
\toprule
Material & State & $J=0$ & $J=2$ & $J=4$ & Other\\
\midrule
\sampleTMHD{} & $^7F_0$ & 95.550741 & 2.001675 & 2.416704 & 0.030880\\
              & $^5D_0$ & 99.860533 & 0.010667 & 0.128204 & 0.000596\\
\addlinespace
\sampleBA{}   & $^7F_0$ & 98.815049 & 0.650869 & 0.533219 & 0.000863\\
              & $^5D_0$ & 99.972383 & 0.004107 & 0.023232 & 0.000278\\
\bottomrule
\end{tabular}
\end{table}

Both optical states remain predominantly $J=0$. The largest admixture occurs
in the \sampleTMHD{} $^7F_0$ state, which contains approximately
$2.00\%$ $J=2$ character and $2.42\%$ $J=4$ character.


The hyperfine terms were then restored, and the complete Hamiltonian in
Eq.~\eqref{eq:total-hamiltonian} was diagonalized. For each of the $^7F_0$
and $^5D_0$ manifolds, the six eigenstates having the largest weight in the
corresponding $J=0\otimes|M_I\rangle$ subspace were selected and projected
onto this nuclear-spin basis.

The doublets $g_1$, $g_2$, and $g_3$ belong to the $^7F_0$ manifold, whereas
$e_1$, $e_2$, and $e_3$ belong to the $^5D_0$ manifold; within each manifold,
they are ordered by increasing energy. In the principal-axis frame of the
corresponding total effective quadrupole tensor, the $+$ member of each
time-reversal doublet was expanded in the basis
$\{|M_I=+5/2\rangle,|M_I=-3/2\rangle,|M_I=+1/2\rangle\}$.
The $-$ member follows by time reversal. Overall phases were chosen so that
the coefficient of largest magnitude is positive. The coefficients are
wavefunction amplitudes rather than state populations.

For \sampleTMHD{}, the normalized nuclear components are
\begin{equation}
\begin{aligned}
\lvert\Psi_{g_1,\pm}^{(n)}\rangle
 &= 0.9964\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.0139\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.0837\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{g_2,\pm}^{(n)}\rangle
 &= -0.0371\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.9583\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.2832\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{g_3,\pm}^{(n)}\rangle
 &= -0.0763\lvert M_I=\pm\tfrac{5}{2}\rangle
  - 0.2853\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.9554\lvert M_I=\pm\tfrac{1}{2}\rangle,\\[0.4ex]
\lvert\Psi_{e_1,\pm}^{(n)}\rangle
 &= 0.9992\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.0034\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.0410\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{e_2,\pm}^{(n)}\rangle
 &= -0.0098\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.9875\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.1574\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{e_3,\pm}^{(n)}\rangle
 &= -0.0400\lvert M_I=\pm\tfrac{5}{2}\rangle
  - 0.1577\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.9867\lvert M_I=\pm\tfrac{1}{2}\rangle.
\end{aligned}
\label{eq:nuclear-mixing-tmhd}
\end{equation}

For \sampleBA{}, the corresponding nuclear components are
\begin{equation}
\begin{aligned}
\lvert\Psi_{g_1,\pm}^{(n)}\rangle
 &= 0.0888\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.3237\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.9420\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{g_2,\pm}^{(n)}\rangle
 &= -0.0513\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.9460\lvert M_I=\mp\tfrac{3}{2}\rangle
  - 0.3202\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{g_3,\pm}^{(n)}\rangle
 &= 0.9947\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.0199\lvert M_I=\mp\tfrac{3}{2}\rangle
  - 0.1006\lvert M_I=\pm\tfrac{1}{2}\rangle,\\[0.4ex]
\lvert\Psi_{e_1,\pm}^{(n)}\rangle
 &= 0.9871\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.0449\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.1537\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{e_2,\pm}^{(n)}\rangle
 &= -0.1035\lvert M_I=\pm\tfrac{5}{2}\rangle
  + 0.9112\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.3987\lvert M_I=\pm\tfrac{1}{2}\rangle,\\
\lvert\Psi_{e_3,\pm}^{(n)}\rangle
 &= -0.1222\lvert M_I=\pm\tfrac{5}{2}\rangle
  - 0.4095\lvert M_I=\mp\tfrac{3}{2}\rangle
  + 0.9041\lvert M_I=\pm\tfrac{1}{2}\rangle.
\end{aligned}
\label{eq:nuclear-mixing-ba}
\end{equation}
Within the normalized $J=0$ projection, these nuclear components multiply
the corresponding $^7F_0$ or $^5D_0$ electronic singlet. The associated
eigenvalues give the zero-field hyperfine splittings compared in the following
subsection. The branching ratios were calculated separately from the complete
projected eigenvectors expressed in a common coordinate basis.

\subsection{Zero-field hyperfine structure}

The calculated and experimental hyperfine level schemes are compared in
Fig.~\ref{fig:hyperfine-levels}, and the consecutive splittings are listed in
Table~\ref{tab:hf-results}. The \sampleTMHD{} hyperfine residuals have an RMS
value of \SI{1.14}{\mega\hertz}; the \sampleBA{} residuals have an RMS value
of \SI{1.48}{\mega\hertz}.

\begin{figure}[H]
  \centering
  \includegraphics[width=0.88\textwidth]{hyperfine_level_comparison.pdf}
  \caption{Experimental and calculated zero-field hyperfine level schemes for
  the $^7F_0$ ground and $^5D_0$ excited manifolds. Each scheme is referenced
  to its lowest hyperfine doublet. Numerical labels give the consecutive
  doublet splittings in MHz.}
  \label{fig:hyperfine-levels}
\end{figure}

\begin{table}[H]
\centering
\caption{Experimental and calculated consecutive zero-field hyperfine
splittings. Residuals are calculated minus experimental.}
\label{tab:hf-results}
\begin{tabular}{llS[table-format=2.1]S[table-format=2.2]S[table-format=+1.2]}
\toprule
Material & Manifold and interval & {Exp. (MHz)} & {Calc. (MHz)} & {Residual (MHz)}\\
\midrule
\sampleTMHD{} & $^7F_0$: $g_2-g_1$ & 34.8 & 34.91 & +0.11\\
       & $^7F_0$: $g_3-g_2$ & 20.5 & 22.13 & +1.63\\
       & $^5D_0$: $e_2-e_1$ & 73.8 & 72.46 & -1.34\\
       & $^5D_0$: $e_3-e_2$ & 37.9 & 38.73 & +0.83\\
\addlinespace
\sampleBA{} & $^7F_0$: $g_2-g_1$ & 21.5 & 23.28 & +1.78\\
       & $^7F_0$: $g_3-g_2$ & 34.0 & 33.89 & -0.11\\
       & $^5D_0$: $e_2-e_1$ & 46.2 & 44.22 & -1.98\\
       & $^5D_0$: $e_3-e_2$ & 37.9 & 39.17 & +1.27\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Effective quadrupole contributions}

Table~\ref{tab:q-contributions} gives the effective rank-two contributions
extracted using the common-frame procedure in Section~\ref{sec:q-method}. For
each material and manifold, the isolated tensors are reported in the
principal-axis frame defined by the corresponding total tensor. The inclusion
of $E$ retains the rhombic information required for the $C_1$ Eu sites.

\begin{table}[H]
\centering
\caption{Calculated contributions to the effective zero-field quadrupole
Hamiltonians. All values are in MHz. The $D$ and $E$ values for each isolated
term are expressed in the principal-axis frame of $Q_{\mathrm{tot}}$ for the
same material and manifold.}
\label{tab:q-contributions}
\small
\setlength{\tabcolsep}{7pt}
\begin{tabular}{ll
S[table-format=+2.4]S[table-format=+1.4]
S[table-format=+2.4]S[table-format=+1.4]}
\toprule
& & \multicolumn{2}{c}{$^7F_0$} & \multicolumn{2}{c}{$^5D_0$}\\
\cmidrule(lr){3-4}\cmidrule(l){5-6}
Material & Contribution & {$D$ (MHz)} & {$E$ (MHz)} & {$D$ (MHz)} & {$E$ (MHz)}\\
\midrule
\sampleTMHD{} & $Q_{\mathrm{pq}}$  & +0.0284 & +0.0060 & +0.0004 & -0.0001\\
       & $Q_{4f}$            & +6.0575 & +0.6872 & +0.3969 & -0.0627\\
       & $Q_{\mathrm{lat}}$ & -15.1678 & +0.7385 & -18.7058 & +1.4855\\
       & $Q_{\mathrm{tot}}$ & -9.0818 & +1.4316 & -18.3085 & +1.4227\\
\addlinespace
\sampleBA{} & $Q_{\mathrm{pq}}$  & -0.0171 & -0.0238 & +0.0004 & -0.0000\\
       & $Q_{4f}$            & -1.9367 & -2.5597 & +0.2087 & -0.0036\\
       & $Q_{\mathrm{lat}}$ & +10.8985 & +4.2727 & -12.4553 & +3.4936\\
       & $Q_{\mathrm{tot}}$ & +8.9446 & +1.6892 & -12.2462 & +3.4900\\
\bottomrule
\end{tabular}
\end{table}

The complete five-component tensor was retained in the calculation; the
numbers in Table~\ref{tab:q-contributions} are its $D$--$E$ representation,
not independent fitted parameters. The tensor non-additivity
$\|\mathbf Q_{\mathrm{tot}}-\mathbf Q_{\mathrm{pq}}-
\mathbf Q_{4f}-\mathbf Q_{\mathrm{lat}}\|_{\mathrm F}$ was at most
\SI{1.46e-4}{\mega\hertz}, confirming a numerically consistent decomposition
at the reported precision. The largest difference between the eigenvalues of
the projected six-state Hamiltonian and its rank-two effective representation
was \SI{1.52e-4}{\mega\hertz}. The effective $D$--$E$ model therefore
reproduces the calculated zero-field hyperfine spectrum far more closely than
the experimental uncertainty relevant here.

\subsection{Hyperfine-state branching ratios}

Rows of the branching matrices correspond to the three $^7F_0$ ground-state
hyperfine doublets and columns to the three $^5D_0$ excited-state doublets.
Each matrix element is the row-normalized transition strength defined by
Eqs.~\eqref{eq:doublet-strength} and \eqref{eq:branching-ratio}. The
experimental and calculated matrices are
\begin{align}
P^{\mathrm{exp}}(\sampleTMHD{})&=
\begin{pmatrix}
0.856&0.108&0.036\\
0.132&0.636&0.232\\
0.012&0.256&0.732
\end{pmatrix}, &
P^{\mathrm{calc}}(\sampleTMHD{})&=
\begin{pmatrix}
0.857&0.107&0.036\\
0.133&0.636&0.231\\
0.010&0.257&0.733
\end{pmatrix},
\label{eq:branching-509}\\[1ex]
P^{\mathrm{exp}}(\sampleBA{})&=
\begin{pmatrix}
0.936&0.055&0.009\\
0.055&0.900&0.045\\
0.009&0.045&0.946
\end{pmatrix}, &
P^{\mathrm{calc}}(\sampleBA{})&=
\begin{pmatrix}
0.936&0.054&0.010\\
0.055&0.900&0.045\\
0.009&0.046&0.945
\end{pmatrix}.
\label{eq:branching-520}
\end{align}
The RMS matrix-element residual for \sampleTMHD{} is 0.00109. For
\sampleBA{}, it is 0.00045. The corresponding maximum absolute residuals are
0.00213 and 0.00075, respectively.

Overall, the selected Hamiltonians reproduce the branching ratios accurately
and give MHz-level agreement with the four zero-field hyperfine splittings.
The \sampleBA{} optical constraints are also reproduced closely. The larger
optical residuals of \sampleTMHD{} and the uncertain weak spectral features
show that its crystal-field parameter set remains underconstrained.

\subsection{Discussion}

This limitation is primarily experimental rather than numerical.
Phenomenological crystal-field models are designed to work with extensive
sets of assigned spectroscopic levels, which provide independent constraints
on both the energies and wavefunctions. For example, Guillot-No{"e}l
\textit{et al.} used 42 experimental levels in their analysis of
$\mathrm{Pr}^{3+}{:}\mathrm{La}_2(\mathrm{WO}_4)_3$
\cite{guillot2010calculation}. In a complete Eu$^{3+}$ treatment, Smith
\textit{et al.} used 61, 15, and 30 experimental crystal-field levels for the
$C_{4v}$, $C_{3v}$, and $C_2$ sites, respectively. Their refinement also
sampled the hyperfine splittings for 100 magnetic-field directions at
\SI{400}{\milli\tesla}, where such data were available
\cite{smith2022complete}. In the present materials, several expected
crystal-field components cannot yet be assigned confidently, so the fitted
energies do not fully constrain the corresponding wavefunctions. In addition,
the available hyperfine constraints consist of zero-field splittings and
branching ratios, without spectra measured as a function of magnetic-field
magnitude and orientation. More complete optical level assignments together
with field-dependent hyperfine spectroscopy would constrain the state mixing
and tensor orientations independently. Thus, the two most direct routes to
improving the present fits are (i) identifying and assigning more optical
crystal-field levels and (ii) measuring the hyperfine spectra while sweeping
the magnetic-field magnitude and orientation. We expect these additional
spectroscopic constraints to improve both the accuracy and the uniqueness of
the fitted crystal-field description substantially.

% \color{blue}
% Write a summary of the crystal field calculation, which will be in the main texts:

% To obtain a theoretical description of the Eu(III) molecular platform, we performed crystal-field calculations for the two materials studied here. The model combines the observed crystal-field levels, zero-field hyperfine splittings, and hyperfine-state branching ratios within a single Hamiltonian, thereby connecting the molecular coordination environment to the measured spectroscopic properties. The calculated eigenvectors provide consistent assignments of the electronic and nuclear-spin character of the relevant \(^{7}F_{0}\) and \(^{5}D_{0}\) states, including their \(J\)-mixing and hyperfine-state composition. This description is particularly relevant because chemical modification of the coordination environment offers a possible route for controlling the hyperfine-level structure required for quantum-memory protocols. Although additional assigned optical levels and magnetic-field-dependent hyperfine spectra would further constrain the model, the fitted Hamiltonian establish a quantitative reference for these materials and provide a physically informed starting point for interpreting future measurements and evaluating chemically modified Eu(III) molecular systems.
% \color{black}

